Risk measures based on weak optimal transport

In this paper, we study convex risk measures with weak optimal transport penalties. In a first step, we show that these risk measures allow for an explicit representation via a nonlinear transform of the loss function. In a second step, we discuss computational aspects related to the nonlinear transform as well as approximations of the risk measures using, for example, neural networks. Our setup comprises a variety of examples, such as classical optimal transport penalties, parametric families of models, uncertainty on path spaces, moment constrains, and martingale constraints. In a last step, we show how to use the theoretical results for the numerical computation of worst-case losses in an insurance context and no-arbitrage prices of European contingent claims after quoted maturities in a model-free setting.

==> preamble.tex <==
\usepackage[T1]{fontenc}  % codifica font
\usepackage[utf8]{inputenc}  % lettere accentate
\usepackage[english]{babel} % document language

% margin settings
\usepackage[a4paper,hmargin=3cm,vmargin=3.5cm,heightrounded]{geometry}
\usepackage{xcolor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages:                                %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage[colorlinks=True,linkcolor=blue,urlcolor=blue]{hyperref} %% for coloring bibliography citations and linked URLs
\RequirePackage{graphicx} %% for including figures
\usepackage{mathrsfs} % implements \mathscr
\usepackage[font=scriptsize,labelfont={scriptsize}]{subfig} % implements \subfloat
\usepackage{bbm} % implements \mathbbm
\usepackage{enumerate}
\usepackage{caption} % captions personalization
\captionsetup{tableposition=top,figureposition=bottom,font=small}
\usepackage{comment}
%\usepackage{todonotes}
%\setlength{\marginparwidth}{2cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Math environments and settings:          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\numberwithin{equation}{section}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{assumptions}[theorem]{Assumptions}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% My definitions:                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% greek letters
\newcommand{\eps}{\varepsilon}
%\renewcommand{\rho}{\varrho}
\renewcommand{\phi}{\varphi}

%% sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\renewcommand{\S}{\mathbb{S}}

%% probability symbols
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}


% calligraphic letters
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

% mathscript letters
\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}

% mathbf letters
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\boldsymbol{t}}

% mathfrak letters
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fk}{\mathfrak{k}}

%% more mathematical letters and abbreviations
\renewcommand{\d}{{\rm d}}
\newcommand{\cpl}{{\rm Cpl}}
\newcommand{\mart}{{\rm Mart}}
\renewcommand{\ker}{{\rm Ker}}
\newcommand{\Lip}{{\rm Lip}}
\newcommand{\dom}{{\rm dom}}
\newcommand{\pr}{{\rm pr}}
\newcommand{\Rd}{{\R^d}}
\def\Ck{{{\rm C}_\kappa}}
\def\Cb{{{\rm C}_{\rm b}}}
\def\Cbi{{{\rm C}_{\rm b}^\infty}}
\def\lscb{{\rm LSC}_{\rm b}}
\def\Bm{{{\rm B}}}
\def\Bb{{{\rm B}_{\rm b}}}
\newcommand{\one}{\mathbbm{1}} % mathbbm version
\newcommand{\ba}{{\rm ba_+}}
\newcommand{\ca}{{\rm ca_+^1}}

%% maths operator
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\df}{{\rm D}_\phi}
\DeclareMathOperator{\dfh}{{\rm D}_{\phi_h}}
\DeclareMathOperator{\prj}{pr}
\DeclareMathOperator{\ex}{ex}

% people review commands
\newcommand{\as}[1]{{\textcolor{red}{ #1}}}

% paper related commands
\newcommand{\pen}{c}

